Understanding the Performance and Estimating the Cost of LLM Fine-Tuning

Due to the cost-prohibitive nature of training Large Language Models (LLMs), fine-tuning has emerged as an attractive alternative for specializing LLMs for specific tasks using limited compute resources in a cost-effective manner. In this paper, we characterize sparse Mixture of Experts (MoE) based LLM fine-tuning to understand their accuracy and runtime performance on a single GPU. Our evaluation provides unique insights into the training efficacy of sparse and dense versions of MoE models, as well as their runtime characteristics, including maximum batch size, execution time breakdown, end-to-end throughput, GPU hardware utilization, and load distribution. Our study identifies the optimization of the MoE layer as crucial for further improving the performance of LLM fine-tuning. Using our profiling results, we also develop and validate an analytical model to estimate the cost of LLM fine-tuning on the cloud. This model, based on parameters of the model and GPU architecture, estimates LLM throughput and the cost of training, aiding practitioners in industry and academia to budget the cost of fine-tuning a specific model.

==> 2_motivations.tex <==
\section{Motivations}
\label{section:Motivation}
Training an LLM from scratch is both time-consuming and resource-demanding. Finetuning is a light-weight way to tune a pretrained general-purpose LLM model, and make it suitable for domain-specific tasks. MoE is another technique that splits the large network into sub-networks (called experts), and selectively applies a subset of them to reduce computation. There is a lack of an understanding of how the sparsity in the MoE model affects the performance of both the model and the hardware it runs on. In this work, we investigate the model accuracy, runtime, and GPU characteristics of LLM model fine-tuning. As depicted in Fig.~\ref{fig:overview}, we compare how different LLM models (\ballnumber{1}) perform across various inputs (\ballnumber{2}), and with different fine-tuning sparsity setups (\ballnumber{3}). We also do an ablation study to show how they change with various sequence sizes, batch sizes, and models. We also parse the results in different granularity, i.e. high-level, layer-level, and kernel-level. We give insights that will guide LLM model development, finetuning setups, and hardware development.   
